Study of e/gamma trigger for the electron calibration stream

This note describes a study of the possibilities for selecting an electron calibration stream using the High level electron trigger (Level 2 and the event filter). Using the electromagnetic calorimeter reconstruction and the track reconstruction algorithms, an evaluation has been performed of the selection efficiencies and purities for different physics channels with single or double electrons in the final state. A study of the calibration stream composition, including the background from QCD processes, is presented.

==> bibliografia.tex <==
\begin{thebibliography}
\bibitem{athena}  nome, \emph{titolo} 
\bibitem{c++}  nome, \emph{titolo} 
\bibitem{ipatrec}  nome, \emph{titolo} 
\bibitem{muid}  nome, \emph{titolo} 
\bibitem{spect}  nome, \emph{titolo} 
\bibitem{muonbox}  nome, \emph{titolo} 
\bibitem{ptdr}  nome, \emph{titolo} 
%\bibitem{nome}  nome, \emph{titolo} 
\end{thebibliography}



==> doccut.tex <==
\section{Moore}
Moore (Muon Object Oriented Reconstruction) is a track reconstruction 
package for the Muon Spectrometer. 
A detailed description of Moore is available elsewhere~\cite{Moore}.
 
Moore takes as input collections of digits or clusters inside the 
Muon Spectrometer (CSC, MDT, RPC, TGC)  and outputs 
fitted reconstructed tracks whose parameters are referred 
at the first measured point of the Muon Spectrometer.
 
The reconstruction is performed in several steps and each step is 
driven by an ATHENA top-Algorithm module (MooMakeXXX).
% see Figure~\ref{fig:Mooscheme}.  
%\begin{figure}[tp]
%\begin{center}
%\epsfig{file=moorescheme.eps,width=\textwidth}
%\caption[]{Data access from the Moore Algorithms.}
%\label{fig:Mooscheme}
%\end{center}
%\end{figure}
Each algorithm is independent, i.e. it retrieves objects created 
by the previous modules from StoreGate and it builds a
transient object to be recorded in StoreGate where it is available 
for the subsequent algorithms. 
The only link between algorithms are the transient objects, in such a way that the 
algorithms depend on transient objects but transient objects do not
depend on algorithms. 
The decoupling between data and algorithms and the natural step 
sequence of algorithm performing the reconstruction gives
the opportunity to plug-in different reconstruction algorithms at 
run time.

As it is now the overall reconstruction starts from the searches for $\phi$ 
regions of activity and builds PhiSegments (MooMakePhiSegments). For each  
$\phi$-Segment, the associated MDTs are found and a {\it crude}
 RZSegment is built (this is essentially a collection of z hits) 
(MooMakeRZSegments).

Inside the MDTs the drift distance is calculated from the drift time, 
by applying various corrections: such as the TOF, the second coordinate, 
the propagation along the wire, the Lorenz effect.
From the 4 tangential lines the best one is found.
All the MDT segments of the outer station are combined with 
those of the Middle layer.
The MDT hits of each combination are added to the phi-hits of the $\phi$ 
Segment, forming outer track candidates. 
All the successfully fitted candidates are kept for further processing 
(MooMakeRoads).

The successfull outer track is subsequentely used to associate 
inner station MDT hits. A final track is defined as a successfully 
fitted collection of trigger hits and MDT hits from at least 
two layers (MooMakeTracks). 
The parameters of the fitted track are referred to the first measured 
point of the Muon Spectrometer.

When dealing with data already selected by the trigger the first two steps
(MooMakePhiSegments) and (MooMakeRZSegments) can be substitute with {\it ad  
hoc} makers that seed the track search in the regions selected by the trigger.
  



==> headings.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 
%                                                                     %
% Macintosh:     Macintosh HD:Paolo:/u1/pvalente/tesi2e/headings.tex  %
%                                                                     %
% HP-UX hpserver:                   /u1/pvalente/tesi2e/headings.tex  %
%                                                                     %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%                                                                     %
%                 Tesi di Laurea di Paolo Valente                     %  
%                                                                     %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\makeatletter
%\renewcommand{\chaptermark}[1]{\markboth{{\bf\large\@chapapp\ \thechapter .\ } #1}}
\renewcommand{\chaptermark}[1]{\markboth{#1}{}} 
\renewcommand{\sectionmark}[1]{\markright{\bf\large\thesection\ #1}}
\makeatother

\lhead[\fancyplain{}{\bf\large\thepage}]{\fancyplain{}{\it\large\rightmark}}
\rhead[\fancyplain{}{\it\large\leftmark}]{\fancyplain{}{\bf\large\thepage}}
\lfoot{\fancyplain{\bf\large\thepage}{}}



==> headings1.tex <==
\makeatletter
\renewcommand{\chaptermark}[1]{\markboth{{} #1}}
%                                     {{} #1}} 
\renewcommand{\sectionmark}[1]{\markright{{\bf\large\thesection\ } #1}}
%\makeatother

\lhead[\fancyplain{}{\bf\large\thepage}]{\fancyplain{}{\it\large\rightmark}}
\rhead[\fancyplain{}{\it\large\leftmark}]{\fancyplain{}{\bf\large\thepage}}
\cfoot{\fancyplain{\bf\large\thepage}{}}


==> hyphenations.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 
%                                                                     %
% HP-UX hpserver:/nfs/kloe02/kloe08/data/users/sciascia/tesi/tesi.tex %
%                                                                     %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%                                                                     %
%                 Tesi di Laurea di Barbara Sciascia                  %  
%                                                                     %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\hyphenation{par-ti-cel-la par-ti-cel-le ele-men-ta-re ele-men-ta-ri}
\hyphenation{vio-la-zio-ne co-me con-se-guen-za quin-di han-no stra-nez-za}
\hyphenation{dop-piet-to dop-piet-ti de-ca-di-men-to de-ca-di-men-ti}
\hyphenation{con-ser-va-zio-ne si-mil-men-te co-niu-ga-zio-ne}
\hyphenation{se-mi-le-pto-ni-co se-mi-le-pto-ni-ci lep-to-ni-ci}
\hyphenation{ha-mil-to-nia-na au-to-sta-to au-to-sta-ti}
\hyphenation{so-vrap-po-si-zio-ne so-vrap-po-si-zio-ni}
\hyphenation{con-fi-gu-ra-zio-ne con-fi-gu-ra-zio-ni}
\hyphenation{tran-si-zio-ne tran-si-zio-ni piom-bo}
\hyphenation{spe-ri-men-ta-le spe-ri-men-ta-li spe-ri-men-tal-men-te}
\hyphenation{con-si-de-ra-re in-te-ra-zio-ne in-te-ra-zio-ni}
\hyphenation{cor-re-zio-ne cor-re-zio-ni mas-sa piom-bo}
\hyphenation{in-tro-dot-to in-tro-dot-ta in-tro-dot-ti in-tro-dot-te}
\hyphenation{pos-so-no es-se-re que-stio-ne}
\hyphenation{es-pri-me-re es-pres-sio-ne es-pres-sio-ni}
\hyphenation{es-pres-so es-pres-si es-pres-sa es-pres-se}
\hyphenation{in-tro-du-zio-ne in-ter-pre-ta-to in-ter-pre-ta-ti}
\hyphenation{for-ma-li-smo for-ma-li-smi her-mi-tia-no her-mi-tia-ni}
\hyphenation{coor-di-na-ta coor-di-na-te coef-fi-cien-te coef-fi-cien-ti}
\hyphenation{de-ter-mi-na-re ot-te-ne-re im-ma-gi-na-rio}
\hyphenation{im-ma-gi-na-rio im-ma-gi-na-ri im-ma-gi-na-ria im-ma-gi-na-rie} 
\hyphenation{la-scian-do evi-den-te-men-te na-tu-ral-men-te}
\hyphenation{Ha-mil-to-nia-na sta-ti ca-na-li co-mu-ni in-ter-fe-ren-za}
\hyphenation{cam-pio-na-tu-ra pro-ble-ma u-san-do mol-te-pli-ci-ta}
\hyphenation{io-niz-za-zio-ne io-niz-za-re u-sa-to}
\hyphenation{in-di-vi-du-are ci-ne-ma-ti-ci}
\hyphenation{con-si-de-ran-do con-te-nu-ti vo-lu-me fi-du-cia-le}
\hyphenation{dis-cre-te de-fi-ni-to ef-fi-cien-za co-stru-zio-ne}
\hyphenation{ca-me-ra de-ri-va e-spe-ri-men-to que-sto ca-pi-to-lo}
\hyphenation{mac-chi-na u-ni-co in-for-ma-zio-ni pro-ve-nien-ti}
\hyphenation{ac-cu-ra-tez-za fo-to-me-tro ca-li-bra-zio-ne re-la-zio-ni}
\hyphenation{de-ter-mi-na-zio-ne in-va-rian-za mi-su-ra pro-du-zio-ne}
\hyphenation{tar-ghet-ta de-di-ca-to mo-du-lo con-tie-ne som-ma-ti}
\hyphenation{piat-ti ge-o-me-tri-ca ri-ge-ne-ra-to spe-ri-men-ta-zio-ne}


==> macros.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 
%                                                                     %
% Macintosh:     Macintosh HD:Paolo:/u1/pvalente/tesi2e/macros2e.tex  %
%                /scrtch1/kloe/barbara/tesi/BLaurea                   %
% HP-UX hpserver:                   /u1/pvalente/tesi2e/macros2e.tex  %
%                                                                     %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%                                                                     %
%                 Tesi di Laurea di Barbara Sciascia                  %  
%                                                                     %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\makeatletter
\def\fnum@figure{{\bf Figura \thefigure}\footnotesize}
\def\fnum@table{{\bf Tabella \thetable}\footnotesize}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\@chapapp{Capitolo}

\def\@makechapterhead#1{\vspace*{50\p@}
%        \vspace*{50\p@}
  {\parindent \z@ \centering \reset@font
    \ifnum \c@secnumdepth >\m@ne
      \LARGE\bfseries \@chapapp{} \thechapter 
      \par
     \vskip 20\p@
   \fi
   \Huge \bfseries #1\par
    \nobreak
    \vskip 40\p@
  }}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\newcommand{\chaptermark}[1]{\markboth{\thechapter. #1}{}}
%\newcommand{\sectionmark}[1]{\markright{\thesection. #1}}









%\def\@schapter#1{\if@twocolumn
%                  \@topnewpage[\@makeschapterhead{#1}]%
%                 \else
%                   \@makeschapterhead{#1}%
%                   \@afterheading
%                 \fi}
%\def\@makeschapterhead#1{%
%  \vspace*{50\p@}%
%  {\parindent \z@ \centering
%    \reset@font
%    \Huge \bfseries  #1\par
%    \nobreak
%    \vskip 40\p@
% }}
%
\def\tableofcontents{\@restonecolfalse\if@twocolumn\@restonecoltrue\onecolumn
  \fi\chapter*{Indice\@mkboth {\bf {Indice}} {\bf{Indice}}}
  \@starttoc{toc}\if@restonecol\twocolumn\fi}
%
\def\thebibliography#1{\chapter*{Bibliografia\addcontentsline{toc}{chapter}
  {Bibliografia}\@mkboth
  {\bf Bibliografia}{\bf Bibliografia}}\list
  {[\arabic{enumi}]}{\settowidth\labelwidth{[#1]}\leftmargin\labelwidth
    \advance\leftmargin\labelsep
    \usecounter{enumi}}
    \def\newblock{\hskip .11em plus .33em minus -.07em}
    \sloppy
    \sfcode`\.=1000\relax}
%
\makeatother
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\scr                 {\scriptstyle}
\def\sscr                {\scriptscriptstyle}
\def\rmscr               {\rm \scriptstyle}
\def\rmsscr              {\rm \scriptscriptstyle}

%

\newcommand{\e}[1]       {\mbox{$\cdot 10^{\sscr #1} $}}
\newcommand{\Darrow}     {\mbox{\rlap{$\leftarrow$}\raisebox{0.6ex}{$\rightarrow$}}}
\newcommand{\bra}[1]     {\mbox{$\langle #1|$}}
\newcommand{\ket}[1]     {\mbox{$| #1\rangle$}}
\newcommand{\Bra}[1]     {\mbox{$\left\langle #1\right|$}}
\newcommand{\Ket}[1]     {\mbox{$\left| #1\right\rangle$}}
\newcommand{\braket}[3]  {\mbox{$\langle #1|#2|#3\rangle$}}
\newcommand{\Braket}[3]  {\mbox{$\left\langle #1\left|#2\right|#3\right\rangle$}}
\newcommand{\scalare}[2]  {\mbox{$\langle #1|#2\rangle$}}
\newcommand{\Scalare}[2]  {\mbox{$\left\langle #1\left|#2\right\rangle$}}
\newcommand{\slashed}[1] {\mbox{\rlap{\hbox{/}}#1}}
\newcommand{\GIm}[1]     {\Im{\frak{m}\left(#1\right)}}
\newcommand{\GRe}[1]     {\Re{\frak{e}\left(#1\right)}}
\newcommand{\duplet}[2]  {\left({\rlap{\raisebox{-1.5ex}{#2}}
                          \raisebox{1.5ex}{#1}}\right)}
\newcommand{\triplet}[3]  {\left({\rlap{\raisebox{-2.0ex}{#3}}
                          \raisebox{0ex}{#2}}{\raisebox{2.0ex}{#1}}\right)}			  
			  
%
\newcommand{\taumeno}    {\mbox{${\tau}^{\sscr -}$}}
\newcommand{\nutau}      {\mbox{${\nu}_{\sscr \tau}$}}
\newcommand{\zzero}      {\mbox{${\rm Z}^{\sscr 0}$}}
\newcommand{\zalf}      {\mbox{${\rm Z}^{\sscr {\alpha}}$}}
\newcommand{\epiu}      {\mbox{${\rm e}^{\sscr +}$}}
\newcommand{\emeno}     {\mbox{${\rm e}^{\sscr -}$}}
\newcommand{\mupiu}     {\mbox{${\mu}^{\sscr +}$}}
\newcommand{\mumeno}    {\mbox{${\mu}^{\sscr -}$}}
\newcommand{\mumenopiu} {\mbox{$\mu^{\sscr \mp}$}}
\newcommand{\emenopiu}  {\mbox{${\rm e}^{\sscr \mp}$}}
\newcommand{\pmenopiu}  {\mbox{${\pi}^{\sscr \mp}$}}
\newcommand{\mupiumeno} {\mbox{$\mu^{\sscr \pm}$}}
\newcommand{\epiumeno}  {\mbox{${\rm e}^{\sscr \pm}$}}
\newcommand{\ppiumeno}  {\mbox{${\pi}^{\sscr \pm}$}}
\newcommand{\nue}       {\mbox{${\nu}_{\rm\sscr e}$}}
\newcommand{\numu}      {\mbox{${\nu}_{\sscr \mu}$}}
\newcommand{\ppiu}   {\mbox{${\pi}^{\rmsscr +} $}}
\newcommand{\pmeno}  {\mbox{${\pi}^{\rmsscr -} $}}
\newcommand{\pzero}  {\mbox{${\pi}^{\rmsscr 0} $}}
\newcommand{\kpiu}   {\mbox{${\rm K}^{\rmsscr +} $}}
\newcommand{\kmeno}  {\mbox{${\rm K}^{\rmsscr -} $}}
\newcommand{\kzero}  {\mbox{${\rm K}^{\rmsscr 0} $}}
\newcommand{\kzerob} {\mbox{${\bar{\rm K}}^{\rmsscr 0} $}}
\newcommand{\bzero}  {\mbox{${\rm B}^{\rmsscr 0} $}}
\newcommand{\bzerob} {\mbox{${\bar{\rm B}}^{\rmsscr 0} $}}
\newcommand{\kl}     {\mbox{${\rm K}^{\rmsscr 0}_{\rmsscr L} $}}
\newcommand{\ks}     {\mbox{${\rm K}^{\rmsscr 0}_{\rmsscr S} $}}

\newcommand{\GammaS} {\Gamma_{\rm\sscr S}}
\newcommand{\GammaL} {\Gamma_{\rm\sscr L}}
\newcommand{\gammaS} {\gamma_{\rm\sscr S}}
\newcommand{\gammaL} {\gamma_{\rm\sscr L}}

\newcommand{\kuno}   {\mbox{${\rm K}^{\rmsscr 0}_{\rmsscr 1} $}}
\newcommand{\kdue}   {\mbox{${\rm K}^{\rmsscr 0}_{\rmsscr 2} $}}
\newcommand{\kzerokzerob} {\ensuremath{\kzero - \kzerob}}
\newcommand{\MS}          {\mbox{$\cal MS$}}
\newcommand{\La}          {\mbox{${\cal L}$}}
\newcommand{\CP}          {\ensuremath{\mbox{$\cal CP$}}}
\newcommand{\T}           {\mbox{$\cal T$}}
\newcommand{\CPT}         {\ensuremath{\mbox{$\cal CPT$}}}
\newcommand{\C}           {\mbox{$\cal C$}}
\newcommand{\Pa}          {\mbox{$\cal P$}}
\newcommand{\Hsuno}    {\mbox{${\cal H}_{\sscr |\Delta S|=1}$}} 
\newcommand{\Hsdue}    {\mbox{${\cal H}_{\sscr |\Delta S|=2}$}}
\newcommand{\imez}     {\mbox{$\frac{\scr i}{\rm\scr 2}$}}
\newcommand{\unotre}    {\mbox{$\sqrt{\frac{\rm\sscr 1}{\rm\sscr 3}}$}}
\newcommand{\duetre}    {\mbox{$\sqrt{\frac{\rm\sscr 2}{\rm\sscr 3}}$}}
\newcommand{\kls}       {\mbox{${\rm K}^{\rmsscr 0}_{\rmsscr L,S} $}}
\newcommand{\phifa}      {$\phi$-{\it factory\/}}   
\newcommand{\Da}         {DA$\Phi$NE}
\newcommand{\epiuemeno}  {\mbox{${\rm e}^{\sscr +} {\rm e}^{\sscr -}$}}

\newcommand{\lsim}   {\mbox{\rlap{\raisebox{-1ex}{$\sim$}}$<$}}
\newcommand{\gsim}   {\mbox{\rlap{\raisebox{-1ex}{$\sim$}}$>$}}

\newcommand{\Me}     {\mbox{${\rm CH}_{\sscr 4}$}}
\newcommand{\iso}    {\mbox{$i{\rm C}_{\sscr 4}{\rm H}_{\sscr 10}$}}
\newcommand{\CO}     {\mbox{${\rm CO}_{\sscr 2}$}}

\newcommand{\epseps} {\mbox{$\frac{\epsilon{\rm\sscr '}}{\epsilon}$}}
\newcommand{\eps}    {\mbox{$\epsilon{\rm\sscr '}$}}

% Paolo Valente





==> monica.tex <==
%\if@twoside
%\def\ps@headings{\let\@mkboth\markboth
%\def\@oddfoot{\tensf\thepage}\def\@evenfoot{}
%\def\@evenhead{\rule[-8pt]{\texwidth}{0.5pt}\hskip-\texwidth
%{\tensf \thepage}\hfil {\tensf\leftmark}}
%\def\@oddhead{\rule[-8pt]{\texwidth}{0.5pt}\hskip-\texwidth
%{\sl \rightmark}\hfil {\tensf\thepage}}
%\def\chaptermark##1{\markboth {{ifnum \c@secnumdepth >\m@ne
%   \@chaapp\ \it\thechapter. \ \fi##1}}{}}
%\def\sectionmark##1{\markright {{ifnum \c@secnumdepth >\z@
%    \@thesection. \ \ fi ##1}}}}

%\fancyhead{}
\fancyhf{}
\renewcommand{\chaptermark}[1]{\markboth{\thechapter. #1}{}}
\renewcommand{\sectionmark}[1]{\markright{\thesection. #1}{}}
\lhead[\bfseries\sl{\rightmark}]{\bf \sl{ ATLAS}}
\rhead[\bf \sl{Tesi di Laurea }]{\bfseries\sl\footnotesize{\leftmark}}
%\lfoot[\bfseries\thepage]{}
%\rfoot[]{\bfseries\thepage}
\cfoot[\thepage]{\thepage}  

    
    
    
\newcommand{\Jn}   {\mbox{${\rm J}^{\rmsscr N}_{\rmsscr{\alpha } $}}}
\newcommand{\Jcp}  {\mbox{${\rm J}^{\rmsscr {C+}}_{\rmsscr{\alpha }} $}}
\newcommand{\Jc}   {\mbox{${\rm J}^{\rmsscr C}_{\rmsscr{\alpha } $}}}
\newcommand{\Jem}  {\mbox{${\rm J}^{\rmsscr {em}}_{\rmsscr{\alpha } $}}}

\newcommand{\A}    {\mbox{${\rm A}^{\rmsscr{\alpha } } $}}
\newcommand{\co}  {\mbox{${\cos{\theta}_{w}} $}} 
\newcommand{\se}  {\mbox{${\sin{\theta}_{w}} $}}
\newcommand{\Wp}  {\mbox{${\rm W}^{\rmsscr {+{\alpha}}} $}}
\newcommand{\Wm}  {\mbox{${\rm W}^{\rmsscr {-{\alpha}}} $}}
\newcommand{\W}  {\mbox{${\rm W}^{\rmsscr {\pm}} $}}

\newcommand{\bnumu}      {\mbox{${\bar{\nu}}_{\sscr \mu}$}}
\newcommand{\bnue}       {\mbox{${\bar{\nu}}_{\rm\sscr e}$}}
\newcommand{\bnutau}     {\mbox{${\bar{\nu}}_{\sscr \tau}$}}








